Robust-by-Design Classification via Unitary-Gradient Neural Networks

The use of neural networks in safety-critical systems requires safe and robust models, due to the existence of adversarial attacks. Knowing the minimal adversarial perturbation of any input x, or, equivalently, knowing the distance of x from the classification boundary, allows evaluating the classification robustness, providing certifiable predictions. Unfortunately, state-of-the-art techniques for computing such a distance are computationally expensive and hence not suited for online applications. This work proposes a novel family of classifiers, namely Signed Distance Classifiers (SDCs), that, from a theoretical perspective, directly output the exact distance of x from the classification boundary, rather than a probability score (e.g., SoftMax). SDCs represent a family of robust-by-design classifiers. To practically address the theoretical requirements of a SDC, a novel network architecture named Unitary-Gradient Neural Network is presented. Experimental results show that the proposed architecture approximates a signed distance classifier, hence allowing an online certifiable classification of x at the cost of a single inference.

==> distancefull.tex <==
\begin{tabular}{lccc}
\textbf{Models} &   \textbf{LB/MAP} & \textbf{\#N} & \textbf{Box.C.}\\
\midrule
LConvNet (raw)        &  $79.0\pm0.26$ &  $12345$ & \checkmark \\
LipConvNet5  (raw)    &  $78.0\pm0.26$ &  $12345$ & \checkmark \\
ResNet9 (raw)         &  $78.7\pm0.22$ &  $12345$ & \checkmark \\
LConvNet (norm)       &  $79.0\pm0.26$ &  $12345$ & \checkmark \\
LipConvNet5 (norm)    &  $78.0\pm0.26$ &  $12345$ & \checkmark \\
ResNet9 (norm)        &  $78.7\pm0.22$ &  $12345$ & \checkmark \\
LConvNet (raw)        &  $79.0\pm0.26$ &  $12345$ &  \\
LipConvNet5  (raw)    &  $78.0\pm0.26$ &  $12345$ &  \\
ResNet9 (raw)         &  $78.7\pm0.22$ &  $12345$ &  \\
LConvNet (norm)       &  $79.0\pm0.26$ &  $12345$ &  \\
LipConvNet5 (norm)    &  $78.0\pm0.26$ &  $12345$ &  \\
ResNet9 (norm)        &  $78.7\pm0.22$ &  $12345$ &  \\
\midrule
MaxMin+orth (norm)        &  $79.0\pm0.26$ &  $12345$ &  \checkmark\\
OPLU+upd (raw)        &  $79.0\pm0.26$ &  $12345$ & \checkmark \\
MaxMin+orth (norm)        &  $79.0\pm0.26$ &  $12345$ &  \\
OPLU+upd (raw)        &  $79.0\pm0.26$ &  $12345$ & \\

MaxMin+upd (norm)        &  $79.0\pm0.26$ &  $12345$ &  \\
OPLU+upd (norm)        &  $79.0\pm0.26$ &  $12345$ &  \\
OPLU+orth (norm)        &  $79.0\pm0.26$ &  $12345$ &  \\
\bottomrule
\end{tabular}

==> img/distance.tex <==
\begin{tabular}{lccl}
\toprule
                  \textbf{Model} &  \textbf{LB/MAP} &  \textbf{\#N} & \textbf{B.C} \\
\midrule
                  ResNet9 (norm) & $.21\!\pm\!.042$ &          7900 &       \cmark \\
                   ResNet9 (raw) & $.34\!\pm\!.063$ &          6669 &       \cmark \\
             LargeConvNet (norm) & $.36\!\pm\!.036$ &          2148 &       \cmark \\
              LipConvNet5 (norm) & $.41\!\pm\!.060$ &          7838 &       \cmark \\
              LargeConvNet (raw) & $.46\!\pm\!.057$ &          7219 &       \cmark \\
               LipConvNet5 (raw) & $.58\!\pm\!.069$ &          6911 &       \cmark \\
  \textbf{UGNN+OPLU+updB (norm)} & $.67\!\pm\!.129$ &          7101 &       \cmark \\
   \textbf{UGNN+Abs+updB (norm)} & $.67\!\pm\!.129$ &          7220 &       \cmark \\
  \textbf{UGNN+OPLU+updU (norm)} & $.67\!\pm\!.131$ &          7281 &       \cmark \\
   \textbf{UGNN+Abs+updU (norm)} & $.67\!\pm\!.128$ &          7244 &       \cmark \\
\textbf{UGNN+MaxMin+updU (norm)} & $.67\!\pm\!.130$ &          7311 &       \cmark \\
\textbf{UGNN+MaxMin+updB (norm)} & $.69\!\pm\!.109$ &          4386 &       \cmark \\
   \textbf{UGNN+OPLU+updU (raw)} & $.70\!\pm\!.090$ &          7125 &       \cmark \\
   \textbf{UGNN+OPLU+updB (raw)} & $.70\!\pm\!.093$ &          7098 &       \cmark \\
 \textbf{UGNN+MaxMin+updB (raw)} & $.71\!\pm\!.087$ &          7114 &       \cmark \\
 \textbf{UGNN+MaxMin+updU (raw)} & $.71\!\pm\!.088$ &          7118 &       \cmark \\
    \textbf{UGNN+Abs+updB (raw)} & $.71\!\pm\!.090$ &          6960 &       \cmark \\
    \textbf{UGNN+Abs+updU (raw)} & $.71\!\pm\!.092$ &          6940 &       \cmark \\
                  ResNet9 (norm) & $.26\!\pm\!.036$ &          7904 &       \xmark \\
                   ResNet9 (raw) & $.44\!\pm\!.056$ &          6663 &       \xmark \\
             LargeConvNet (norm) & $.44\!\pm\!.027$ &          7933 &       \xmark \\
              LipConvNet5 (norm) & $.52\!\pm\!.031$ &          7840 &       \xmark \\
              LargeConvNet (raw) & $.58\!\pm\!.046$ &          2429 &       \xmark \\
               LipConvNet5 (raw) & $.74\!\pm\!.049$ &          6912 &       \xmark \\
   \textbf{UGNN+OPLU+updU (raw)} & $.93\!\pm\!.101$ &          6755 &       \xmark \\
   \textbf{UGNN+OPLU+updB (raw)} & $.95\!\pm\!.063$ &          7102 &       \xmark \\
 \textbf{UGNN+MaxMin+updU (raw)} & $.95\!\pm\!.061$ &          7127 &       \xmark \\
 \textbf{UGNN+MaxMin+updB (raw)} & $.95\!\pm\!.056$ &          7117 &       \xmark \\
    \textbf{UGNN+Abs+updB (raw)} & $.95\!\pm\!.058$ &          6965 &       \xmark \\
    \textbf{UGNN+Abs+updU (raw)} & $.95\!\pm\!.058$ &          6949 &       \xmark \\
  \textbf{UGNN+OPLU+updB (norm)} & $.96\!\pm\!.046$ &          7215 &       \xmark \\
   \textbf{UGNN+Abs+updB (norm)} & $.96\!\pm\!.049$ &          7228 &       \xmark \\
  \textbf{UGNN+OPLU+updU (norm)} & $.96\!\pm\!.047$ &          7282 &       \xmark \\
\textbf{UGNN+MaxMin+updU (norm)} & $.96\!\pm\!.051$ &          7316 &       \xmark \\
\textbf{UGNN+MaxMin+updB (norm)} & $.96\!\pm\!.044$ &          7327 &       \xmark \\
   \textbf{UGNN+Abs+updU (norm)} & $.96\!\pm\!.039$ &          7247 &       \xmark \\
\bottomrule
\end{tabular}

